Data-efficient Domain Randomization with Bayesian Optimization

When learning policies for robot control, the required real-world data is typically prohibitively expensive to acquire, so learning in simulation is a popular strategy. Unfortunately, such polices are often not transferable to the real world due to a mismatch between the simulation and reality, called 'reality gap'. Domain randomization methods tackle this problem by randomizing the physics simulator (source domain) during training according to a distribution over domain parameters in order to obtain more robust policies that are able to overcome the reality gap. Most domain randomization approaches sample the domain parameters from a fixed distribution. This solution is suboptimal in the context of sim-to-real transferability, since it yields policies that have been trained without explicitly optimizing for the reward on the real system (target domain). Additionally, a fixed distribution assumes there is prior knowledge about the uncertainty over the domain parameters. In this paper, we propose Bayesian Domain Randomization (BayRn), a black-box sim-to-real algorithm that solves tasks efficiently by adapting the domain parameter distribution during learning given sparse data from the real-world target domain. BayRn uses Bayesian optimization to search the space of source domain distribution parameters such that this leads to a policy which maximizes the real-word objective, allowing for adaptive distributions during policy optimization. We experimentally validate the proposed approach in sim-to-sim as well as in sim-to-real experiments, comparing against three baseline methods on two robotic tasks. Our results show that BayRn is able to perform sim-to-real transfer, while significantly reducing the required prior knowledge.

==> plots/eval_sim2sim_2row1col.tex <==
%/home/fmrt/Software/SimuRLacra/Pyrado/data/perma/experiments/qq-su/bayrn-power_qq_sub_sim2sim/2020-10-08_15-39-59--rand-Mp-Mr
\begin{subfigure}[t]{\columnwidth}%{0.495\columnwidth}
	\begin{tabular}{p{0.75\columnwidth} p{0.23\columnwidth}}
		\vspace{0pt}\input{plots/gp_posterior_ret_mean_hm.pgf} &
		\vspace{0pt}\hspace{-5pt}\input{plots/gp_posterior_ret_mean_cb.pgf}
	\end{tabular}
	\caption{\vspace*{-0.1\baselineskip}posterior mean}
	\label{fig_sim_eval_QQ_mean}
\end{subfigure}%
\\[0.5\baselineskip]
\begin{subfigure}[t]{\columnwidth}%{0.495\columnwidth}{0.49\linewidth}
	\begin{tabular}{p{0.75\columnwidth} p{0.23\columnwidth}}
		\vspace{0pt}\input{plots/gp_posterior_ret_std_hm.pgf} &
		\vspace{0pt}\hspace{-5pt}\input{plots/gp_posterior_ret_std_cb.pgf}
	\end{tabular}
	\caption{\vspace*{-0.1\baselineskip}posterior standard deviation}	
	\label{fig_sim_eval_QQ_std}
\end{subfigure}%

==> tables/bayrn_argmax_QQ_WAM.tex <==
\begin{tabular}{lll}
	\rowcolor{gray!50}
	\textbf{Estimate}       & \textbf{\sub}                & \textbf{\bic} \\
	% QQ
%	$\domdistrparams_{\text{MAP}}$ & $[0.023, \num{2.54e-7}, 0.094, \num{1.52e-6}, 0.151, \num{5.31e-5}, 0.069, \num{8.43e-7}]$ & \\%2020-09-06_16-02-55--rand-Mp-Mr-Lp-Lr
%	$\domdistrparams_{\text{MAP}}$ (means only) & $[0.023, 0.094, 0.151, 0.069]$ & \\%2020-09-06_16-02-55--rand-Mp-Mr-Lp-Lr
%	$\domdistrparams_{\text{MAP}}$ (means only) & $[0.020, 0.091, 0.143, 0.082]$ & \\%2020-09-08_16-02-01--rand-Mp-Mr-Lp-Lr
	$\domdistrparams_{\text{MAP}}$ (means only) & $[0.023, 0.090, 0.147, 0.078]$ & $[0.312, \num{4.50e-5}, 0.021, 0.032, 0.389]$\\%2020-10-02_19-39-39--rand-Mp-Mr-Lp-Lr_lower-std AND 2020-09-16_13-47-09--rand-rl-rd-bm-js-jd
	% WAM
%	$\domdistrparams_{\text{nominal}}$ & $[0.024, 0, 0.095, 0, 0.129, 0, 0.085, 0]$ & $[0.3, 0, \num{2e-4}, 0, 0.020, 0, 4, 0, 5, 0]$\\
	$\domdistrparams_{\text{nominal}}$ (means only) & $[0.024, 0.095, 0.129, 0.085]$ & $[0.300, \num{2.00e-4}, 0.020, 0.050, 0.200]$\\
\end{tabular}
